AgentDroid: A Multi-Agent Framework for Detecting Fraudulent Android Applications

With the increasing prevalence of fraudulent Android applications such as fake and malicious applications, it is crucial to detect them with high accuracy and adaptability. We present AgentDroid, a novel tool for Android fraudulent application detection based on multi-modal analysis and multi-agent systems. AgentDroid overcomes the limitations of traditional detection methods such as the inability to handle multimodal data and high false alarm rates. It processes Android applications and extracts a series of multi-modal data for analysis. Multiple LLM-based agents with specialized roles analyze the relevant data and collaborate to detect complex fraud effectively. We curated a dataset containing various categories of fraudulent applications and legitimate applications and validated our tool on this dataset. Experimental results indicate that our multi-agent tool based on GPT-4o achieves an accuracy of 91.7% and an F1-Score of 91.68%, outperforming the baseline methods. A video of AgentDroid is available at https://youtu.be/YOM9Ex-nBts.

==> Limitation.tex <==
\section{Limitation}

Firstly, the dataset used in this study is relatively small, containing only 660 APK samples. This limitation in sample size may not fully represent the diversity of real-world applications, thereby affecting the generalizability and reliability of the research findings.

Secondly, the baseline methods selected in this paper also have certain limitations. Although these methods have been widely used in previous studies, they are relatively outdated.

To address these limitations, we will expand the size and diversity of the dataset to enhance the generalization ability of the conclusions. Additionally, incorporating more state-of-the-art baseline methods, such as those based on advanced algorithms, would allow for a more comprehensive evaluation of the framework's performance.
